Unbiased Loss Functions for Multilabel Classification with Missing Labels

This paper considers binary and multilabel classification problems in a setting where labels are missing independently and with a known rate. Missing labels are a ubiquitous phenomenon in extreme multi-label classification (XMC) tasks, such as matching Wikipedia articles to a small subset out of the hundreds of thousands of possible tags, where no human annotator can possibly check the validity of all the negative samples. For this reason, propensity-scored precision -- an unbiased estimate for precision-at-k under a known noise model -- has become one of the standard metrics in XMC. Few methods take this problem into account already during the training phase, and all are limited to loss functions that can be decomposed into a sum of contributions from each individual label. A typical approach to training is to reduce the multilabel problem into a series of binary or multiclass problems, and it has been shown that if the surrogate task should be consistent for optimizing recall, the resulting loss function is not decomposable over labels. Therefore, this paper derives the unique unbiased estimators for the different multilabel reductions, including the non-decomposable ones. These estimators suffer from increased variance and may lead to ill-posed optimization problems, which we address by switching to convex upper-bounds. The theoretical considerations are further supplemented by an experimental study showing that the switch to unbiased estimators significantly alters the bias-variance trade-off and may thus require stronger regularization, which in some cases can negate the benefits of unbiased estimation.

==> macros.tex <==
\NewDocumentCommand{\wrapbraces}{m}{\left\{ #1 \right\}}
\NewDocumentCommand{\wrapbrackets}{m}{\left[ #1 \right]}
\NewDocumentCommand{\wrapparens}{m}{\left( #1 \right)}

% Default font settings
\ProvideDocumentCommand{\spacefont}{m}{\ensuremath{\mathcal{\MakeUppercase{#1}}}}
\ProvideDocumentCommand{\functionalfont}{m}{\ensuremath{\mathds{\MakeUppercase{#1}}}}
\ProvideDocumentCommand{\vectorfont}{m}{\ensuremath{\mathbf{\MakeLowercase{#1}}}}
\ProvideDocumentCommand{\matrixfont}{m}{\ensuremath{\mathbf{\MakeUppercase{#1}}}}

\NewDocumentCommand{\DeclareFunctional}{smmm}{
    % #1 : star operator
    % #2 : command name
    % #3 : symbol
    % #4 : delimiters
    \NewDocumentCommand{#2}{e{_^}o}{
        \IfBooleanTF{#1}{
            \def\basesymbol{\operatorname*{\functionalfont{#3}}}
        }{
            \def\basesymbol{\operatorname{\functionalfont{#3}}}     
        }
        % ##1 : subscript
        % ##2 : superscript
        % ##3 : argument
        \def\decorated{\basesymbol\IfNoValueTF{##1}{}{_{##1}}\IfNoValueTF{##2}{}{^{##2}}}
        \IfNoValueTF{##3}{\decorated}{\decorated\!#4{##3}}
    }
}


==> parts/simdata.tex <==
%!TEX root = ../main.tex

We generated artificial data in the following setup: We consider a setting in
which there are 100 different labels, which are independent and where each has
a probability of 10\%. We randomly draw ground-truth samples, and generate
observed samples by removing labels according to a propensity $p$ which we set
the same for all labels. Finally, we generate predictions by choosing a
random label from the ground truth. 

We draw $n \in \set{10^4, 10^5}$ such samples and calculate the average
per-example recall, which corresponds to a recall@1 since we constructed the
prediction such that there is always one predicted label. We repeat this
process $m=1000$ times in order to gather statistics to calculate the variance
of the estimator, and we do this for a range of different propensity values.

\begin{figure}
    \centering
    \input{plots/simdata}
    \caption{Unbiased estimate of per-example recall with artificial 
    data as described in the main text. For the biased estimate, the
    difference between $n=10^4$ and $n=10^5$ is not noticeable, so only one
    curve has been plotted. The shaded region corresponds to one standard
    deviation, the dotted black line denotes the true recall.
}
    \label{fig:simdata}
\end{figure}

The results visualized in \autoref{fig:simdata} show that for propensities
lower than $0.4$, the estimates variance becomes too large. We have also
calculated a biased estimate, by calculating an unbiased estimate of the
numerator (number of correct predictions) and denominator (number of total
labels present) and dividing the result, which results in much lower variance.
In the case of uniform propensities, this is identical to computing vanilla
recall. As the graph shows, for low propensities this estimate becomes
unusable too, as it deviates strongly from the true value. However, for medium
propensity, the unbiased estimator still has little variance, but has
noticeable better accuracy than the biased one, as can be seen in the inset.

Together with \autoref{thm:multi-unique}, these results imply that for large
datasets with very low propensity, unbiased estimates cannot be used to
calculate the per-example recall, and the best any usable estimator can be is
asymptotically unbiased.


==> plots/bce.tex <==
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            vertical sep=0pt,
            y descriptions at=edge left},
        ylabel={frequency},
        xlabel={loss}, ylabel shift = -1em,
        ymax=1300, ymin=0,
        width=0.5\linewidth
    ]
   
    \nextgroupplot[very thick]
        \addplot+[mark=none] table[x=x,y=estimate]{plots/bce_10.txt};
        \addplot+[mark=none] table[x=x,y=ground truth]{plots/bce_10.txt};

        \addplot[mark=none,] coordinates {(-2.222750948289568, 0) (-2.222750948289568, 1300)};
        \addplot[mark=none,] coordinates {(4.225136676896915, 0) (4.225136676896915, 1300)};
        \addplot[mark=none,dashed] coordinates {(-0.3535474689293958, 0) (-0.3535474689293958, 1300)};
        \addplot[mark=none,dashed] coordinates {(2.3559331975367437, 0) (2.3559331975367437, 1300)};

    \nextgroupplot[very thick]
        \addplot+[mark=none] table[x=x,y=estimate]{plots/bce_1000.txt};
        \addplot+[mark=none] table[x=x,y=ground truth]{plots/bce_1000.txt};

        \addplot[mark=none,] coordinates {(0.8434425014458238, 0) (0.8434425014458238, 1300)};
        \addplot[mark=none,] coordinates {(1.1568419491598594, 0) (1.1568419491598594, 1300)};
        \addplot[mark=none,dashed] coordinates {(0.859800176038469, 0) (0.859800176038469, 1300)};
        \addplot[mark=none,dashed] coordinates {(1.1404842745672141, 0) (1.1404842745672141, 1300)};
    \end{groupplot}
\end{tikzpicture}

==> plots/recall.tex <==
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            vertical sep=0pt,
            y descriptions at=edge left},
        ylabel={frequency},
        xlabel={loss}, ylabel shift = -0.5em,
        ymax=1400, ymin=0,
        width=0.5\linewidth,
        height=4.5cm
    ]
   
    \nextgroupplot[very thick]
        \addplot+[mark=none] table[x=x,y=estimate]{plots/recall_4.txt};
        \addplot+[mark=none] table[x=x,y=ground truth]{plots/recall_4.txt};
        \addplot+[mark=none] table[x=x,y=biased]{plots/recall_4.txt};

    \nextgroupplot[very thick]
        \addplot+[mark=none] table[x=x,y=estimate]{plots/recall_6.txt};
        \addplot+[mark=none] table[x=x,y=ground truth]{plots/recall_6.txt};
        \addplot+[mark=none] table[x=x,y=biased]{plots/recall_6.txt};
    \end{groupplot}
\end{tikzpicture}
